Neutrino Emissions of TXS 0506+056 caused by a Supermassive Binary Black Hole Inspiral?

The IceCube neutrino observatory detected two distinct flares of high-energy neutrinos from the direction of the blazar TXS 0506+056: a $\sim 300$ TeV single neutrino on September 22, 2017 and a $3.5\sigma$ signature of a dozen TeV neutrinos in 2014/2015. In a previous work, it was shown that these two episodes of neutrino emission could be due to an inspiral of a supermassive binary black hole (SMBBH) close to its merger at the core of TXS 0506+056. Such an inspiral can lead to quasi-periodic particle emission due to jet precession close to the final coalescence. This model made predictions on when the next neutrino emission episode must occur. On September 18, 2022, IceCube detected an additional, $\sim 170$ TeV neutrino in directional coincidence with the blazar TXS 0506+056, being consistent with the model prediction. Additionally, in April 2021, the Baikal Collaboration reported the detection of a $224\pm 75$ TeV neutrino, with TXS 0506+056 being in the uncertainty range of the event direction. We show that these four distinct flares of neutrino emission from TXS 0506+056 are consistent with a precessing jet scenario, driven by an inspiraling SMBBH. Using improved modeling, we are now able to constrain the total mass together with the mass ratio for the binary. We predict when the next neutrino flares from TXS 0506+056 should be happening. Finally, we estimate the detection potential of the Laser-interferometer Space Antenna (LISA) for the merger in the future.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

